Characterizing Data Scientists in the Real World

Data collection is pervasively bound to our digital lifestyle. A recent study by the IDC reports that the growth of the data created and replicated in 2020 was even higher than in the previous years due to pandemic-related confinements to an astonishing global amount of 64.2 zettabytes of data. While not all the produced data is meant to be analyzed, there are numerous companies whose services/products rely heavily on data analysis. That is to say that mining the produced data has already revealed great value for businesses in different sectors. But to be able to fully realize this value, companies need to be able to hire professionals that are capable of gleaning insights and extracting value from the available data. We hypothesize that people nowadays conducting data-science-related tasks in practice may not have adequate training or formation. So in order to be able to fully support them in being productive in their duties, e.g. by building appropriate tools that increase their productivity, we first need to characterize the current generation of data scientists. To contribute towards this characterization, we conducted a public survey to fully understand who is doing data science, how they work, what are the skills they hold and lack, and which tools they use and need.

==> sec/abs_ing.tex <==
Every day, data is being collected from all different types of sources. According to the company Domo, data is being collected from ad clicks, likes on social media, shares, transactions, streaming content, and so much more. Their study, which focused on how much data is generated on the internet showed that, in 2019, every minute were sent 188.000.000 emails, downloaded 390.030 apps, conducted 4.497.420 searches in Google and, only the American population used 4.416.720GB of internet. Also, a study conducted by the International Data Corporation in 2014, showed that By 2020, there were around 40 zettabytes of data, compared to the 1.2 zettabytes of data in 2010. They also estimated that only 37 \% of all this data collected from surveillance, entertainment, social media, etc., would be a candidate for analysis.
	
This enormous amount of data in itself may not be relevant. The real value of data lies in the information it hides about individuals and the world. As a result, it is more crucial than ever for businesses of all sizes to focus on the data they collect from diverse sources and use the insights they gain to become more competitive in their fields of expertise. In this scenario, companies rely on recruiting professionals to join data science teams capable of gleaning insights and extracting value from data.

Data science, as the name implies, can be seen as the science that studies data. It is a multidisciplinary field where professionals, commonly known as data scientists, transform data into insights and decisions. Several researchers have focused on data science, intending to explain it and demonstrate its value in several contexts. However, in this research study, we shifted the focus to those who practice data science. 

This work aims to take advantage of the information collected through interviews and a public survey to fully understand who is doing data science, how they work, what are the skills they hold and lack, and which tools they need. The main goal is to fully understand how we can assist data science workers being more productive in their jobs, which will allow data science community to propose adequate solutions for these professionals.

==> sec/acronyms.tex <==
%!TEX root = ../dissertation.tex

\newacronym{mei}{MEI}{Mestrado em Engenharia Inform\'{a}tica}
\newacronym{um}{UM}{Universidade do Minho}

==> sec/background.tex <==
Our research contributes to the existing literature on data science and data science workers. In this chapter, we review some concepts surrounding the definition of data science and its applicability to solve real problems. Also, in the last section of this chapter, we mention present some published studies that are related with our work.

\section{Data science}

To understand how data can be used to enable enhanced insight and decision making we have to understand what data science is and how did this field evolved over time.

In 1962, John Tukey, an important figure in the mathematical and statistical worlds, described a new science about learning from data when he wrote that data analysis "is intrinsically an empirical science"~\cite{Donoho201750Science,JohnW.Tukey1962TheAnalysis}. Some years later, Peter Naur, a Danish software programming pioneer, proposed \textit{datalogy}, which he described as ``the science of data and data processes'', as an alternative to computer science. In 1974, he used the term \textit{Data Science} for the first time in one of his books to describe ``the science of dealing with data''~\cite{CraigStedman2021WhatGuide,GilPress2013AScience}. 

From that moment on, several authors started using the term \textit{data science} to refer to the discovery of knowledge from data analysis, always establishing a link with the traditional statistical methodology and modern computer technology. The relationship between the concept of data science and statistics became so important among authors that, in 1996, C. F. Jeff Wu, a university professor of Industrial and Systems Engineering, presented a lecture titled ``\textit{Statistics = Data Science?}'', in which he advocated that statistics be renamed data science and statisticians data scientists~\cite{Donoho201750Science}.

In 2001, after years of being used as an alternative to statistics or computer science, \textit{data science} was finally described as an independent discipline, by William S. Cleveland. In a paper called ``\textit{Data Science: An Action Plan for Expanding the Technical Areas of the field of Statistics}'', Cleveland suggested that data science need to be a new multidisciplinary field that merges the base knowledge of statisticians and computer scientists, to ``produce a powerful force for innovation''~\cite{Donoho201750Science,Kelleher2018DataScience}. Since 2001, the concept of data science has widen beyond that of a redefinition of statistics and became widely used in the next years.

Nowadays, data science is viewed as an amalgamation of classical disciplines like statistics, data mining, databases, and distributed systems. Generally, it involves the application of quantitative and qualitative methods to solve relevant problems and its ultimate goal is to improve decision making~\cite{Provost2013,VanderAalst2016,Waller}.

As suggested in~\cite{DeMauro2018}, a lot of roles are involved in data science, and they can be divided into four categories: Business Analyst (project managers, business analysts, product managers, etc.), Data Scientist (data engineers, data scientists, data analysts, data consultants, etc.), Big Data Developer (software engineers, software developers, etc.), and Big Data Engineer (data architects, system engineers, infrastructure administrators, etc.).

\subsection{Data Science workflow}

Data science projects involve a series of data collection and analysis steps that define a data science workflow or methodology~\cite{Saltz2020WhatWorkflow}. Following a well-defined workflow allows data science professionals to organize their work in an efficient way that ultimately leads to the discovery of new knowledge that can be used to solve real problems~\cite{Logallo2019DataScience}. 

There are several well-known data science methodologies, that vary on the number of steps and in the way to plan tasks, but in every methodology we can identify the following phases \cite{Azevedo2008,Huber2019,Kurgan2006,Olson2008,Rogalewicz2016, Shafique2014}:
    
    \begin{enumerate}
        \item[-] \textit{Business Understanding} - this phase consists of understanding the problem and defining the business goals to be achieved;
        \item[-] \textit{Data Understanding} - this phase consists of collecting and exploring data to identify quality issues that need to be addressed so that the results are good and reliable;
        \item[-] \textit{Data Preparation} - this phase consists of selecting the relevant data and processing it in order to construct the final dataset;
        \item[-] \textit{Data Analysis} - this phase consists of applying different analysis and visualization techniques to the data to obtain new information;
        \item[-] \textit{Results interpretation and Evaluation} -  this phase consists of interpreting and evaluate the results to extract knowledge and to verify if the business objectives were achieved;
        \item[-] \textit{Deployment and Feedback} - this phase consists of organizing, reporting, and presenting the gained knowledge so that it can be used to solve problems.
    \end{enumerate}
    
\subsection{Data Science techniques and use cases}

During data analysis, knowledge discovery is possible due to a very wide range of techniques that can be classified according to the performed tasks \cite{Han2011,Rogalewicz2016}. The most common tasks are:
    
    \begin{itemize}
        \item[-] \textit{Description} - involves describing patterns and trends lying within data \cite{Larose2005,Rogalewicz2016};
        \item[-] \textit{Clustering} - involves grouping records, observations, or cases into classes of similar objects \cite{Han2011,Larose2005,Olson2008,Rogalewicz2016};
        \item[-] \textit{Classification} - involves collecting various attributes together into discernible categories, in order to classify other instances into one of the them \cite{Han2011,Larose2005,Olson2008,Rogalewicz2016};        
        \item[-] \textit{Association} - involves finding existing rules between dependent attributes \cite{Larose2005,Olson2008,Rogalewicz2016};
        \item[-] \textit{Regression} - involves identifying and analyzing the relationship between variables, in order to identify the likelihood of a specific variable, given the presence of other variables \cite{Han2011,Olson2008};
        \item[-] \textit{Prediction} - involves the combination of data mining techniques to analyze past events or instances, in order to predict a future event \cite{Larose2005,Olson2008}.
    \end{itemize}
    
Due to the plethora of data analysis techniques available, data science provides a number of opportunities to businesses from distinct sectors. Table \ref{table:usecases} summarizes some of the most common data science use cases in different sectors.

\begin{table*}[!htb]
\caption{Data science use cases in different business sectors.}
\label{table:usecases}
\begin{center}
\begin{tabular}{lp{8cm}}
\toprule
\textbf{Sector}                                                  & \textbf{Use cases}                                                                                                                                \\\midrule
\begin{tabular}[c]{@{}l@{}}Banking and\\ Insurance\end{tabular} & \begin{tabular}[c]{@{}l@{}}Fraud detection\\ Risk management\\ Costumer segmentation and support\\ Price optimization\end{tabular}                \\\midrule
Telecommunications                                               & \begin{tabular}[c]{@{}l@{}}Price optimization\\ Customer behavior analysis\\ Network optimization\\ Churn prevention\end{tabular}                \\\midrule
Healthcare                                                       & \begin{tabular}[c]{@{}l@{}}Medical image analysis\\ Virtual assistance for patients\\ Disease evolution management\\ Drug discovery\end{tabular} \\\midrule
Retail                                                           & \begin{tabular}[c]{@{}l@{}}Recommendation engines\\ Price optimization\\ Inventory management\\ Customer sentiment analysis\end{tabular}          \\\midrule
\begin{tabular}[c]{@{}l@{}}Energy and \\ Utilities\end{tabular}  & \begin{tabular}[c]{@{}l@{}}Energy management\\ Customer analytics\\ Fraud detection\\ Campaign effectiveness\end{tabular}\\\bottomrule                          
\end{tabular}
\end{center}
\end{table*}
    
\section{Related work}
\input{sec/related}



==> sec/background_old.tex <==
	The main goal of those who work with large amounts of data is the extraction of knowledge. However, before they can even move on to data analysis, they need to ensure that the data is properly preprocessed so that it can be useful.
	
	To clarify the concepts surrounding the data preprocessing and analysis phases, this chapter presents a brief review of the published work on data cleaning and data mining. 

	\section{Data cleaning}
	
	Data is collected from all types of platforms and gadgets \cite{DOMO2019,Holst2019}. Most of it needs to be analyzed by all types of professionals in order to gain new information and knowledge about the part of the world that it represents \cite{Muller}. This means that detecting and repairing data with errors is one of the major challenges in data analytics, and failure to do so can result in unreliable decisions and poor study results \cite{Chu2016,VanDenBroeck2005}. 
	
	Data cleaning, also called data cleansing, wrangling or scrubbing, deals with removing anomalies from a dataset in order to ensure its quality \cite{Chu2016,Kandel2011,Maletic2009,Muller,Rahm2014,Singh2010,VanDenBroeck2005}. This process is typically divided into several phases, including anomalies detection and their removal, that are executed over several iterations until the desired quality criteria are met \cite{Kandel2011,VanDenBroeck2005}.
	
	\subsection{Data cleaning process}
	
	The data cleaning process is usually time-consuming, rigorous and expensive \cite{Kandel2011,Maletic2000,Muller,Muller2019, Zhang2003}. Data scientists spend about most of their time cleaning up data, which includes looking for errors and inconsistencies to eliminate \cite{Kandel2011,Press2016, Ruiz2017, Zhang2003,Muller2019}.
	
	In recent years there has been an effort to automate this task and try to have it performed by people with a deep knowledge of the manipulated data \cite{Maletic2000,Maletic2009,Muller}. These are the most competent people to specify the cleaning process considering four main tasks:
	
	\begin{enumerate}
	    \item \textit{Data auditing} or \textit{Screening phase} - detection through qualitative (integrity constraints, association rules, patterns) and quantitative (statistical methods, outlier detection) methods which kinds of errors and inconsistencies are to be removed \cite{Chu2016, Muller,Rahm2014, VanDenBroeck2005};
	    \item \textit{Workflow specification} or \textit{Diagnostic phase} - specification of a cleaning workflow that must be applied to the dirty data to automatically eliminate all anomalies in the data \cite{Muller,Rahm2014, VanDenBroeck2005};
	    \item \textit{Workflow execution} or \textit{Treating phase} - elimination of the errors and inconsistencies by executing the data cleaning workflow \cite{Muller,Rahm2014, VanDenBroeck2005};
	    \item \textit{Controlling phase} - inspection of the results and evaluation for the need of a new process iteration taking into account a set of quality criteria \cite{Muller}.
	\end{enumerate}
	
	\subsection{Data quality}
	
	The concept of data quality arises with the need to evaluate the quality of data collected from various sources \cite{Askham2013,Muller,Singh2010}. Data quality plays a critical role in all business and governmental applications \cite{Batini2009} because by ensuring that data has quality and manipulating it into a usable "free from error" form, we know we can trust the knowledge we gain through its analysis \cite{Kandel2011}.
	
	Although there is no clear definition, data quality is commonly conceived as \textit{fitness for use} \cite{Knight2005,Wang1996,Zaveri2016} which, most of the time, is assessed through quality criteria, also known as data dimensions \cite{Askham2013,Fox1994,Muller,Singh2010}. 
	
	A data quality criteria can be defined as any feature, characteristic or attribute that can be measured or assessed to determine the quality of data, such as: \textit{completeness, consistency, conformity, validity, accuracy, and integrity} \cite{Askham2013,Batini2009,Fox1994,Knight2005,Muller,Singh2010,Wang1996}. One important aspect regarding data quality criteria is that they are not consensual \cite{Fox1994}. As so, each organization must choose the set of criteria that better reflects their needs. This enforces the less common idea that these quality criteria must be prioritized and organized hierarchically to allow organizations to quantify their need of cleaning for a specific dataset \cite{Muller,Wang1996}. 
	
    Data quality is affected by the number of errors or anomalies found in data due to misspellings during data entry, missing information or other invalid data \cite{Rahm2014}. Since each of them affects a certain set of quality criteria, it is only possible to achieve higher levels of data quality by removing them.
	
	
	\subsection{Data anomalies}
	
	The first step in a data cleansing process is to identify errors that affect its quality \cite{Chu2016, Muller,Rahm2014, VanDenBroeck2005}. While there is no catalog of all possible errors and the best way to resolve them, there are several studies that identify the most common errors in large datasets. These can be divided into two main categories depending on whether or not data is missing.
	
	\textit{Missing data} in a dataset is often a critical situation, as it is never possible to be sure of the actual value that an attribute or record represents. In this case, two situations can happen. The first is the actual lack of the real value, represented by a null value. The other one is the presence of a default value, indicating the possible lack of that value \cite{Kim2003, Muller, Rahm2014, Zhang2003}.
	
	It is even more difficult to identify errors when there is no data missing, as the causes can be very distinct. This category includes errors related to violation of \textit{integrity constraints}, including erroneous data, misspellings and values outsides specific ranges; \textit{contradictions} between values across the dataset; \textit{discrepancies} between the values represented and the predicted formats; \textit{duplicated values}; and other \textit{irregularities} related to non-uniform use of values, units, and abbreviations \cite{Kim2003, Muller, Rahm2014, Zhang2003}.
	

    \section{Data mining}
    
    The explosive growth in stored data has far exceeded the human ability for comprehension \cite{Han2011}. As so, it has generated an urgent need for new techniques and automated tools that can help us in transforming the vast amounts of data into useful information and knowledge \cite{Han2011,Maimon2005}. This has led to the generation of a new field in computer science called \textit{data mining}. 
    
    Data mining, also popularly referred to as \textit{knowledge extraction}, is the automated extraction of patterns representing potential useful knowledge implicitly stored or captured in large amounts of data \cite{Grupe1995,Han2011,Maimon2005,Rogalewicz2016,Kuonen2004}. This is a multidisciplinary field that draws on work from areas including statistics, computer science, artificial intelligence, machine learning, database management and data visualization \cite{Han2011, Rogalewicz2016, Kuonen2004}.
    
    \subsection{Data mining process}
    
    While some view data mining as a merely analytic task, data mining is better defined as an iterative sequence of steps that allows for knowledge discovery \cite{Kuonen2004}. In the last few years, several methodologies were proposed, in the form of scenarios of gathering and preparing data for further analysis, as well as dissemination of results \cite{Rogalewicz2016}.
    
    One of the most accepted methodology around the knowledge discovery community is the \textbf{CR}oss \textbf{I}ndustry \textbf{S}tandard \textbf{P}rocess for \textbf{D}ata \textbf{M}ining (CRISP-DM), which consists of six phases intended to be cyclic \cite{Azevedo2008,Huber2019,Kurgan2006,Olson2008,Rogalewicz2016, Shafique2014}:
    
    \begin{enumerate}
        \item[-] \textit{Business Understanding} - understanding the project objectives and requirements from a business perspective;
        \item[-] \textit{Data Understanding} - data collection and identification of data quality problems;
        \item[-] \textit{Data Preparation} - selection and processing of raw data in order to construct the final dataset;
        \item[-] \textit{Modeling} - selection and implementation of several model techniques;
        \item[-] \textit{Evaluation} - evaluation of the obtained models in order to verify if the business objectives were achieved;
        \item[-] \textit{Deployment} - reporting and application of the knowledge acquired in the construction of appropriate solutions.
    \end{enumerate}
    
    \subsection{Data mining methods}
    
    Discovery of knowledge in large data sets is made possible thanks to a very wide range of data mining methods, or techniques, that can be classified according to the realized tasks \cite{Han2011,Rogalewicz2016}. The most common data mining tasks are:
    
    \begin{itemize}
        \item[-] \textit{Description} - involves describing patterns and trends lying within data \cite{Larose2005,Rogalewicz2016};
        \item[-] \textit{Clustering} - involves grouping records, observations, or cases into classes of similar objects \cite{Han2011,Larose2005,Olson2008,Rogalewicz2016};
        \item[-] \textit{Classification} - involves collecting various attributes together into discernible categories, in order to classify other instances into one of the them \cite{Han2011,Larose2005,Olson2008,Rogalewicz2016};        
        \item[-] \textit{Association} - involves finding existing rules between dependent attributes \cite{Larose2005,Olson2008,Rogalewicz2016};
        \item[-] \textit{Regression} - involves identifying and analyzing the relationship between variables, in order to identify the likelihood of a specific variable, given the presence of other variables \cite{Han2011,Olson2008};
        \item[-] \textit{Prediction} - involves the combination of other data mining techniques to analyze past events or instances, in order to predict a future event \cite{Larose2005,Olson2008}.
    \end{itemize}

==> sec/interviews.tex <==
To gain initial understanding on the people working on data science, several semi-structured interviews were conducted. Semi-structured interviews are a method of gathering information that allows inexperienced researchers to be in contact with people of interest and capture their perceptions, thoughts, and attitudes \cite{Rowley2012,Wohlin2012}. 

In this chapter, we present all the information related to the interviews, from how the data was collected, to how the data was analyzed and the results of the interviews analysis. In the last section, we present the research decision that was taken based on the findings.

\section{Data collection}
Due to the qualitative nature of this interviews, the goal was to interview people with distinct academic and professional backgrounds, who are currently working in data science. To make sure that the conversations with all the participants covered the same topics, the interviews followed a guide developed with the help from a person with experience in data science to make sure that the language was correct and the questions were important in the context of this study. This initial guide (Appendix \ref{guide}) followed the subsequent structure:

\begin{enumerate}[label=(\roman*)]
    \item Academic and professional backgrounds; 
    \item Work and tasks performed;
    \item Data handling techniques;
    \item Tools and programming languages;
    \item General difficulties.
\end{enumerate}

In this work, the non-probabilistic sampling methods \textit{convenience} and \textit{snowball} were used, meaning that responses were obtained from those people who were available and willing to take part, and people they believed would be willing to take part \cite{Kitchenham2002}. All participants had legal age, signed a consent form (Appendix \ref{consent}), and were interviewed on a voluntary and unpaid basis. 

There were a total of eight interviewees: two data analysts, one business intelligence manager, one big data architect and four data scientists. This group is composed of three women and five men who live and work in Portugal, except for one case who lives and works in the UK. Table \ref{tab1} summarizes the information about the interviewees. 

The interviews were conducted in Portuguese and lasted about 30 minutes. The interview with participant P3 was not considered in our analyzes since the participant did not allow us to ask the initially prepared questions.

\begin{table*}[!tb]
\caption{Interviewees information.}
\begin{center}
\begin{tabular}{lllp{2.4cm}p{4.3cm}l}
\toprule
\textbf{ID} & \textbf{Sex} & \textbf{Age} & \textbf{Job Title}            & \textbf{Education Level} & \textbf{Domain}                    \\ \midrule
P1           & F            & 30           & Data Analyst                  & Master, Marketing & Music Management                              \\ \midrule
P2           & M            & 36           & Business Intelligence Manager & Master, Data Analysis and Decision Support Systems & Retail \\ \midrule
P3           & M            & 37           & Big Data \,\, Architect & Bachelor, Math and Computer Science & Software Development \\ \midrule
P4           & M            & 34           & Data Scientist                & PhD, Electrical and Computer Engineering &  Telecommunication      \\ \midrule
P5           & M            & 42             & Data Scientist                & PhD, Data Mining & Virtual Call Center                                   \\ \midrule
P6           & F            & 26           & Data Analyst                  & Master, Mathematics and Computation & Web Development              \\ \midrule
P7           & F            & 32           & Data Scientist                 & Master, Mathematics Engineering & Virtual Call Center        
\\ \midrule
P8           & M            & 32           & Data Scientist                 & PhD, Evolutionary Biology & Telecommunication
\\ \bottomrule
\end{tabular}
\label{tab1}
\end{center}
\end{table*}

\section{Analysis methodology}

The main goal of the qualitative analysis is to derive conclusions that are supported by the collected data. It is also important that the analysis be carried out in parallel with the data collection, to allow researchers to explore different aspects related to the subject~\cite{Wohlin2012}. This meant examining each interview as the interviews were being conducted to see whether new ideas were introduced and if those ideas were worth examining further in subsequent interviews.

The main technique used to analyze the information collected from the interviews was hypothesis generation based on the ideas exchanged with the interviewees. To this end, we used "constant comparisons" and "cross-case analysis" techniques, which meant comparing the information shared by interviewees on various topics to identify recurring themes and verify whether or not their opinions were the same.

\section{Interviews results}
\label{sec:inter_res}

In this section, we present the results obtained from our analysis of the conducted interviews.

\subsection*{Academic background}

As expected, the participants have quite different academic backgrounds, with the most striking cases being participant P1, who graduated in Hotel Management, and participant P2, who graduated in Economics. However, after a few years of experience in data science-related areas, they both felt the need to obtain skills more suitable to this area. Therefore, participant P1 is currently taking a second master's degree in Business Intelligence and Knowledge Management, and participant P2 began a master's degree in Data Analysis and Decision Support Systems, two years after having worked in auditing information systems, as himself stated\footnote{The quotes represent our best translation of the Portuguese statements.}: 

\disse{I had been working in auditing information systems for two years, and at that time I decided that data was `the thing' and I went to get a master's degree in Data Analysis and Decision Support Systems.}{P2}

\subsection*{Performed tasks} 

Regarding their work, we found out that all the participants end up preforming all the tasks in the analysis process such as data collection, cleaning, analysis and reporting of results, which goes along with the findings in~\cite{Muller2019}. However, we realize that the type of analysis they do can be distinct. For example, within the interviewed group, only those who have training in computer science or engineering perform tasks related to the creation of machine learning and deep learning models, as is the case of participants P4 and P5. The remainder dedicate themselves to more a direct analysis, based on statistical parameters such as average, standard deviation, distributions, etc., which ends up fitting more into the profile of a mathematician or statistician. A similar idea was mentioned in~\cite{Harris2013,Kim2016}, as authors said that data scientists from fields such as business and social sciences have strong numerical reasoning skills and are particularly good in using advanced statistical techniques in their analysis.

\subsection*{Data sources and data types}

Regarding the data sources used by this group of professionals, and similarly to what is mentioned in~\cite{Muller2019}, there is a great variety. In addition to the data internally generated by their teams, the use of public data sources is also frequent. Also, the manipulated data is quite different, ranging from customer data, to operational data. 

An aspect which several mentioned was the lack of metrics that would enable the quality of the data to be assessed beforehand. Participant P2 was the only who reported using any form of data quality metrics. In this case, the participant points that the existence of specific metrics is possible because there is a great knowledge about the data, and that if some drastic changes happens, errors end up being easily detected.

\subsection*{Data cleaning process}

In terms of data pre-processing in order to increase data quality, the majority of the participants agree that this is still one of the most time-consuming and laborious tasks, which goes along with the findings in~\cite{Kim2016,Muller2019}. 

\disse{In terms of time, I would say that I spend 80\% of the time cleaning data and only 20\% analyzing it.}{P1}

The only exceptions were participant P5 and participant P7, since they work with audio files, and the pre-processing only involves converting all files to the same format.

\disse{The pre-processing of our data is not difficult. The only thing we do is to convert all files to the same format.}{P5}

In the remaining cases, participants claim that most of the anomalies that affect the quality of the data concern inputs that have been wrongly introduced by humans. Among the most common errors are duplicated records, missing values, inconsistencies in values (e.g. date formats) and outliers.

\subsection*{Data mining process}

In terms of the most used techniques, participants use a wide variety according to the solutions they want to build, ranging from machine learning techniques, such as clustering, prediction, and classification, to more complex deep learning models. These techniques are usually applied with two main and distinct goals: client segmentation and service customization; cost reduction and optimization of internal processes. In~\cite{Kim2016}, several similar observations were made.

\disse{We have projects with a strong emphasis on the customer and the user experience, but the main focus is on internal projects that aim to enhance the quality of our processes and minimize costs.}{P4}

As far as data analysis concerns, all participants report that they do not follow any work methodology. Instead, everyone agrees that the best way to work with data is to adapt to the situations at hand. Even so, all participants agree that analyzing data does not dispense a great knowledge of the data itself and the business in which the problem is inserted.

\subsection*{Tools and programming languages}

Concerning programming languages, we find that in this group of participants there is a great tendency in the use of programming languages such as R and Python, as well as all of the state-of-the-art packages that the two languages provide both for data visualization and data analysis. The choice of which language to use is usually made according to personal preferences and the type of tasks to be performed. In the case of participants P5 and P7, this choice was made as a team so that all elements of the same project used the same technologies. 

Regarding data analysis tools, most participants stated that they do not usually use them in their day-to-day lives since these tools end up limiting their analysis, which does not happen when they produce all the code they need. Even so, participant P1 and the participant P2 reported that a large part of their analysis is done using only \textit{MS Excel} since this software allows for more immediate results.

\subsection*{General difficulties}

When we asked the participants what were the biggest difficulties they felt regarding their work, several situations were mentioned. For participant P1, the difficulties she feels are related to the fact that she has no training in the field of data science, and that was the reason that led her to pursue a master's degree focused on data analysis. For participant P4, the biggest difficulty is the access to quality information, and relevance to the problems in which he works, a difficulty that is shared by several participants in the study referred in~\cite{Muller2019}. 

\disse{I believe that access to quality information and information relevant to our problems is the greatest challenge.}{P4}

\clearpage
For participant P6, the most challenging part of her job is that she is the only person on her team to perform such tasks. She also notes that she often finds it very difficult to convert business problems into data science issues. In fact, in~\cite{Kim2016} the lack of clear problems and questions is also mentioned, as the authors argue that the academic background of a data scientist may have a significant impact on the way they identify important questions.

\disse{In my case, being alone is a big limitation, [\dots], it is very difficult to have the required business expertise to understand what are its needs.}{P6}

On the other hand, participant P8 says that his greatest challenge, after several years of experience, is the development of stable and scalable code, since he has no training in software engineering.

\disse{On a personal level, I think my biggest challenge is to write a stable and scalable code because my training is not very oriented for software engineering.}{P8}

In these conversations, several participants mentioned that there are also difficulties associated with professionals being hired for data science positions that, in reality, should be occupied by other types of professionals. This can be one of the causes that leads to a considerable overlapping amongst several data science roles, as stated in~\cite{Zhang2020}.

\disse{Companies look at the market and, because there is a demand for data scientists, they also want to hire one. However, looking at the job's requirements, their needs would be easily mitigated by other types of professionals.}{P7}

Participant P2 pointed out that it is important to clarify which are the different areas of data science, so that the professionals who wish to work in this field can position themselves correctly in this environment and understand what are the opportunities that meet their aspirations.

\disse{In my opinion, there are two main areas: technological and application data science. The data scientist of the future must know how to put himself in the right area of data science to avoid regretting what (s)he is doing.}{P2}

In general, all participants agree that it is a great advantage to have people with different backgrounds in data science teams because, although some are better suited to certain tasks than others, they all bring different perspectives on the data.

\clearpage
\section{Research decision}

To better understand professionals in data science, and how they work, we conducted interviews with different people who are currently working in this field. We explored several aspects related to their academic background, the jobs they have, the tasks they perform, and the difficulties they experience in their daily lives. 

From this group, we discovered that data science workers with an education background outside computer science often seek complementary training to overcome several limitations they feel they have, and in such cases, the type of analysis they perform is often based on statistical methods. We also found that data science workers identify the lack of metrics to assess the quality of the data they manipulate, and that they believe that recruiting committees often lack a precise understanding of how a data science worker can add value to their teams.

Based on the findings of the interview analysis, a decision was taken to explore in more depth the impact of the academic background and professional experience of data science professionals on the way they perform their jobs. To ensure that the results were relevant, either due to the number of responses or the diversity of participants, we developed a survey that was distributed online, allowing us to reach data science professionals around the world.


==> sec/introduction_old.tex <==
Every day huge amounts of data are created and manipulated to glean insights and extract value~\cite{Holst2019,DOMO2019,Parkins2017,Kubina2015}. This data comes from very diverse sources and is used for all kinds of purposes. According to the results of DOMO's study on the data generated on the most popular platforms in 2019, 188.000.000 emails and 18.100.000 messages were sent every minute, representing an increase of more 5.000.000 messages compared to 2018. Also, in 2019, there was an increase in the number of searches performed in Google, with about 4.500.000 searches conducted every minute~\cite{DOMO2019}. In the aviation area, there were drastic changes too. The development of new technologies has led to the existence of new, more sophisticated aircraft. Forbes magazine reported that, for every flight performed, five to eight terabytes of data are generated regarding the crew, the passengers, the condition of the engines, etc., i.e. 30 times more data than those generated by the previous generation aircraft~\cite{Maire2016}. This growth has had an impact in all different sectors and led the International Data Corporation to estimate that, by 2020, the worldwide data will increase up to 40 zettabytes~\cite{ODriscoll2013, Turner2014}.

Frequently there are being published news regarding attacks to organizations, which data is stolen; complaints from users who feel their privacy have been violated due to improper and unauthorized collection of their information; and recently, offers from companies who are willing to pay their product's users to access their information. The interest in data reflects in its appreciation, making it one of the most valuable resources to organizations. In fact, in May of 2017, the journal \textit{The Economist} published an article stating that oil was no longer the world's most valuable resource, losing that position to data~\cite{Parkins2017}.

Therefore, companies from all industries, realizing the value of their data, are trying to use it to gain some competitive advantage and get ahead of their rivals~\cite{Davenport2012, Grupe1995, Kubina2015, Provost2013, Williams2018}. However, due to the huge variety and volume of data available, as well as the various data analytics solutions, these companies are looking to have in their teams people with great skills in gathering, cleaning and using data~\cite{Davenport2012, Dhar2014, Provost2013}.

This phenomenon led to a buzz around concepts like \textit{Big Data} and \textit{Data Science}~\cite{Dhar2014,Provost2013, VanDenBroeck2005, Waller, Zhang2013}, which are intricately related in a way that one cannot exist without the other.

\bigbreak
Big Data is a term with many different interpretations that emerged as a result of technological developments in various sectors, for example, life and physical sciences, medicine and healthcare, education, retail, government, communication and media~\cite{Manyika2011, Zhang2013}.

When it comes to big data, the size is not the most important aspect to consider. According to Laney~\cite{Laney2001}, when dealing with data we have to take into consideration three important characteristics: \textit{Volume}, \textit{Variety}, and \textit{Velocity}~\cite{Austin2016, Gandomi2015, Laney2001, Wieczorkowski2014}. Although he did not use the term big data, the widely accepted model he used to describe data become known as the "Three V's of Big Data". Based on this model, big data involves a very large volume of data that is being created, stored, and analyzed exponentially faster than at any period in the history of mankind. This data can be in a variety of formats, such as structured (attributes in a database) or unstructured data (images, video footage, audio, handwritten notes).

To understand how data can be used to enable enhanced insight and decision making we have to understand what data science is. Data science can be seen as a set of fundamental principles that support and guide the extraction of knowledge from data~\cite{Provost2013}. 

Because organizations need to be able to use data in a smart way data science is the job of the future and it can be viewed as an amalgamation of classical disciplines like statistics, data mining, databases, and distributed systems~\cite{Provost2013,VanderAalst2016}. Generally, it involves the application of quantitative and qualitative methods to solve relevant problems and its ultimate goal is to improve decision making~\cite{Provost2013,Waller}. Because of that, a data science worker must have a diverse range of skills, and a great domain knowledge, in order to be able to work creatively with their data.

As suggested in~\cite{DeMauro2018}, a lot of roles are involved in data science, and they can be divided into four categories: Business Analyst (project managers, business analysts, product managers, etc.), Data Scientist (data engineers, data scientists, data analysts, data consultants, etc.), Big Data Developer (software engineers, software developers, etc.), and Big Data Engineer (data architects, system engineers, infrastructure administrators, etc.).

==> sec/motivation.tex <==



==> survey/academic.tex <==
\section*{Academic Background}
    
\begin{enumerate}

    \item In which scientific field did you study? 
    
    For each of the following. choose all that apply: Bachelor's Degree, Master's Degree; Doctoral Degree; Professional Degree.
    
    Note: If you did not enroll in any type of degree-program at college or university, skip this question.

    \begin{itemize}
        \item [-] Humanities (arts, law, languages and literature)
        \item [-] Social sciences (anthropology, psychology, political science, sociology)
        \item [-] Natural Sciences (biology, chemistry, physics)
        \item [-] Computer Science or Computer Engineering or Software engineering
        \item [-] Another engineering discipline (civil, electrical, mechanical)
        \item [-] Mathematics or statistics
        \item [-] Medicine and Health Science (Nursing, pharmacy)
        \item [-] Business (accounting, finance, marketing)
        \item [-] Other

    \end{itemize}
    
    \item Have you ever used other methods for learning data science such as on-line courses, bootcamps, or other non-degree programs? If so, please give a small description (e.g. name, type, duration).
    
\end{enumerate}

==> survey/demographic.tex <==
\section*{Demographic questions} 

\begin{enumerate}
    
    \item What gender do you identify as? (Choose one)
    
    \begin{itemize}
        \item [-] Male
        \item [-] Female
        \item [-] Other
        \item [-] Prefer not to answer.
    \end{itemize}

    \item What is your age? (Choose one)
    
    \begin{itemize}
        \item [-] Younger than 18 years old
        \item [-] 18 - 25 years old
        \item [-] 26 - 30 years old
        \item [-] 31 - 45 years old
        \item [-] 46 - 55 years old
        \item [-] Older than 55 years old
        \item [-] Prefer not to answer.
    \end{itemize}

    \item Where are you currently working? (Choose one)
    
    \begin{itemize}
        \item [-] List of countries
    \end{itemize}
\end{enumerate}

==> survey/evaluation.tex <==
\section*{Self-evaluation}

\begin{enumerate}
    \item Rate your strengths in each of the following tasks. 

    For each of the following, choose one: Very Poor - Little or no knowledge/expertise; Poor - Experimental/vague knowledge; Ok - Familiar and competent user; Good - Regular and confident user; Very Good - Leading expert
    
    \begin{itemize}
        \item[-] Translating business problems to data science problems
        \item[-] Collecting data
        \item[-] Assessing the quality of data
        \item[-] Filtering relevant attributes
        \item[-] Extracting new attributes
        \item[-] Cleaning data
        \item[-] Applying data visualization techniques
        \item[-] Applying classical statistical methods
        \item[-] Applying data mining techniques
        \item[-] Applying deep learning techniques
        \item[-] Evaluating results to respond to business problems / find business opportunities
        \item[-] Transmitting acquired knowledge
    \end{itemize}    
\end{enumerate}






==> survey/professional.tex <==
\section*{Professional Situation}
    
\begin{enumerate}
    
    \item What is your current employment status? (Choose one)
    
    \begin{itemize}
        \item [-] Employed Full-Time
        \item [-] Employed Part-Time
        \item [-] Unemployed 
        \item [-] Freelancer
        \item [-] Retired
        \item [-] Other
        \item [-] Prefer not to answer.
    \end{itemize}
    
    \item How many years of professional experience in data science do you have? (Choose one)
    
    \begin{itemize}
        \item [-] Less than 2 years
        \item [-] 2 - 4 years
        \item [-] 5 - 9 years
        \item [-] 10 - 14 years
        \item [-] 15 - 19 years
        \item [-] 20 - 24 years
        \item [-] 25 - 29 years
        \item [-] 30 - 34 years
        \item [-] 35 - 39 years
        \item [-] 40 - 44 years
        \item [-] 45 - 49 years
        \item [-] 50 years or more
    \end{itemize}
    
    \item Which of the following best describes your current job? (Choose one)
    
    \begin{itemize}
        \item [-] Data Scientist
	    \item [-] Machine Learning Engineer
        \item [-] Software Developer/Engineer
        \item [-] Database Administrator
        \item [-] Data Analyst
        \item [-] Educator or Academic Researcher
        \item [-] Business Analyst
        \item [-] Computer Scientist
        \item [-] Programmer
        \item [-] Statistician
        \item [-] Consultant
        \item [-] Other

    \end{itemize}

    \begin{comment}
    \item In which sector do you work in? (Choose one)
    
    \begin{itemize}
        \item [-] Agriculture
        \item [-] Mining         
        \item [-] Manufacturing         
        \item [-] Energy         
        \item [-] Water and waste management         
        \item [-] Construction         
        \item [-] Transport         
        \item [-] Accommodation and food services         
        \item [-] Media         
        \item [-] Data and information systems         
        \item [-] Finance and insurance services         
        \item [-] Real estate         
        \item [-] Professional services         
        \item [-] Scientific and market research         
        \item [-] Business administration services 
        \item [-] Tourism         
        \item [-] Public administration and defense
        \item [-] Education         
        \item [-] Human health and social work         
        \item [-] Arts, recreation and entertainment     
        \item [-] Consumer services         
        \item [-] Government and public sector         
        \item [-] Wholesale and retail
        \item [-] Other
    \end{itemize}        
    \end{comment}
    
    \item How satisfied are you with your current job? (Choose one)
    
    \begin{itemize}
        \item [-] Extremely satisfied
        \item [-] Slightly satisfied
        \item [-] Neutral
        \item [-] Slightly dissatisfied
        \item [-] Extremely dissatisfied
        \item [-] Prefer not to answer.
    \end{itemize}
    
\end{enumerate}


==> survey/questionario.tex <==
\input{survey/academic}
\clearpage
\input{survey/professional}
\input{survey/evaluation}
\input{survey/work}
\input{survey/technology}
\input{survey/demographic}

==> survey/technology.tex <==
\section*{Technology}

\begin{enumerate}
    
    \item Which of the following Integrated Development Environment (IDE) or Editor do you use most? (Check all that apply)
    
    \begin{itemize}
        \item [-] Visual Studio Code
        \item [-] Visual Studio
        \item [-] Notepad++
        \item [-] Sublime Text
        \item [-] IntelliJ
        \item [-] Eclipse
        \item [-] Atom
        \item [-] PyCharm
        \item [-] Xcode
        \item [-] NetBeans
        \item [-] IPython/Jupyter
        \item [-] RStudio
        \item [-] Emacs
        \item [-] Spyder
        \item [-] Matlab
        \item [-] Vim
        \item [-] Other
        \item [-] None
    \end{itemize}
    
    \item Which of the following Programming, Scripting or Markup Language do you use the most? (Check all that apply) 
    
   \begin{itemize}
        \item [-] Python
        \item [-] R
        \item [-] Scala
        \item [-] Java
        \item [-] C/C++
        \item [-] CSS
        \item [-] Visual Basic
        \item [-] SQL
        \item [-] JavaScript
        \item [-] Matlab
        \item [-] Kotlin
        \item [-] Rust
        \item [-] Bash
        \item [-] PHP
        \item [-] Go
        \item [-] HTML
        \item [-] Other
        \item [-] None
    \end{itemize}

   \item Which of the following Machine Learning Frameworks/Libraries/Tools do you use the most? (Check all that apply)
    
   \begin{itemize}
        \item [-] TensorFlow
        \item [-] Scikit-Learn
        \item [-] Torch/PyTorch
        \item [-] lightgbm
        \item [-] Spark MLlib
        \item [-] Hadoop
        \item [-] Prophet
        \item [-] CNTK
        \item [-] Caret
        \item [-] Xgboost
        \item [-] Mlr
        \item [-] Catboost
        \item [-] Fastai
        \item [-] Theano 
        \item [-] MXNet
        \item [-] Keras
        \item [-] KNIME
        \item [-] H2O
        \item [-] Caffe
        \item [-] Deeplearning4j
        \item [-] Weka
        \item [-] Rapid Miner
        \item [-] Other
        \item [-] None
    \end{itemize}

   \item Which of the following statistics packages/tools do you use the most? (Check all that apply)
    
   \begin{itemize}
        \item [-] Spreadsheet editor (Microsoft Excel, Google Sheets, Numbers, etc)
        \item [-] Tableau
        \item [-] IBM SPSS Statistics
        \item [-] SAS
        \item [-] STATA
        \item [-] Statistica
        \item [-] MatLab (The Mathworks)
        \item [-] Other
        \item [-] None
    \end{itemize}

   \item Which data visualization libraries/tools do you use the most? (Check all that apply)
    
   \begin{itemize}
        \item [-] Tableau
        \item [-] Matplotlib
        \item [-] Seaborn
        \item [-] ggplot2
        \item [-] Plotly
        \item [-] Shiny
        \item [-] D3
        \item [-] Bokeh
        \item [-] Leaflet
        \item [-] Lattice
        \item [-] Geopltlib
        \item [-] Altair
        \item [-] catboost
        \item [-] Mxnet
        \item [-] Keras
        \item [-] H2O
        \item [-] Power Bi
        \item [-] Tableau
        \item [-] Weka
        \item [-] Vega
        \item [-] Highcharts
        \item [-] Google Analytics
        \item [-] Other
        \item [-] None
    \end{itemize}

\end{enumerate}

==> survey/work.tex <==
\section*{Work Characterization}

\begin{enumerate}
        
    \item Which of the following are the most common problems you face at work? 
    
    For each of the following, choose one (if apply): Rarely; Sometimes; Often; Always.
  
    \begin{itemize}
        \item [-] Poor quality data
        \item [-] Difficult access to relevant data
        \item [-] Lack of data science skills
        \item [-] Lack of clear questions to answer
        \item [-] Lack of domain knowledge
        \item [-] Integrating findings into decisions
        \item [-] Expectations of project impact
        \item [-] Results not used by decision makers
        \item [-] Other
        \item [-] None
    \end{itemize}
    
    \item Approximately, what percentage of your time  is spent actively coding? (Choose one)
    
    \begin{itemize}
        \item [-] I don't spend any of my time coding
        \item [-] 1\% - 25\% of the time
        \item [-] 25\% - 50\% of the time
        \item [-] 51\% - 75\% of the time
        \item [-] 76\% - 100\% of the time
    \end{itemize}
    
    \begin{comment}
    \item Which of the following types of data do you use the most? (Check all that apply)
    
    \begin{itemize}
        \item [-] Transaction data
        \item [-] Unstructured data (emails, documents, etc)
        \item [-] Voice/audio data
        \item [-] Image data (video or photo)
        \item [-] Locational/Geospatial data
        \item [-] Time series
        \item [-] Scientific data
        \item [-] Sensor/Device/Machine data
    \end{itemize}    
    \end{comment}
    
    \item What are your analytic goals? (Check all that apply)
    
    \begin{itemize}
        \item [-] Improving customer experience
        \item [-] Retaining customers
        \item [-] Increase sales
        \item [-] Higher quality products or services
        \item [-] More efficient operations
        \item [-] Improving decision making processes
        \item [-] Risk management
        \item [-] Fraud detection or prevention
        \item [-] Medical advancement
        \item [-] Other
    \end{itemize}
    
    \begin{comment}
    \item What is the most important step you would like to take to improve your work? (Choose one)

    \begin{itemize}
        \item [-] Learn new technologies/skills/algorithms
        \item [-] Work on more interesting/important projects
        \item [-] Learn more business skills
        \item [-] Switch companies
        \item [-] Other
        \item [-] None
    \end{itemize}    
    \end{comment}
    
\end{enumerate}


